On the Influence of Shape, Texture and Color for Learning Semantic Segmentation

Recent research has investigated the shape and texture biases of pre-trained deep neural networks (DNNs) in image classification. Those works test how much a trained DNN relies on specific image cues like texture. The present study shifts the focus to understanding the cue influence during training, analyzing what DNNs can learn from shape, texture, and color cues in absence of the others; investigating their individual and combined influence on the learning success. We analyze these cue influences at multiple levels by decomposing datasets into cue-specific versions. Addressing semantic segmentation, we learn the given task from these reduced cue datasets, creating cue experts. Early fusion of cues is performed by constructing appropriate datasets. This is complemented by a late fusion of experts which allows us to study cue influence location-dependent on pixel level. Experiments on Cityscapes, PASCAL Context, and a synthetic CARLA dataset show that while no single cue dominates, the shape + color expert predominantly improves the prediction of small objects and border pixels. The cue performance order is consistent for the tested convolutional and transformer architecture, indicating similar cue extraction capabilities, although pre-trained transformers are said to be more biased towards shape than convolutional neural networks.

==> figures/fusion/fig_expert_pred_carla.tex <==
\centering
\begin{subfigure}[]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/anisodiff_RGB_Town01_0001585.png}
\includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/anisodiff_RGB_Town01_0001591.png}
\includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/anisodiff_RGB_Town01_0002307.png}
\caption*{$\text{shape}_{\text{EED}}$ RGB expert}
\end{subfigure}
\begin{subfigure}[]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/texture_RGB_Town01_0001585.png}
\includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/texture_RGB_Town01_0001591.png}
\includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/texture_RGB_Town01_0002307.png}
\caption*{texture RGB expert}
\end{subfigure}
\begin{subfigure}[position]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/Town01__0001585.png}
\includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/Town01__0001591.png}
\includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/Town01__0002307.png}
\caption*{CARLA ground truth}
\end{subfigure}
\caption[Qualitative results of $\text{shape}_{\text{EED}}$ RGB and texture RGB on CARLA]{Comparison of the prediction of the two CARLA experts $\text{shape}_{\text{EED}}$ RGB (left) and texture RGB (mid). For reference reasons we display the ground truth in the third column (right). More clear predictions of the segment boundaries can be observed for the shape expert. The texture expert however can distinguish between the \textit{sky} and \textit{road} class without difficulty. It predicts more blob-like segments than the shape expert whose predictions are more granular.} \label{fig:visual_carla_experts}

==> figures/fusion/fig_overview_fusion_pred_heat.tex <==
\begin{figure*}[htb]
\centering
    \begin{minipage}{0.6\textwidth}
        \begin{subfigure}[b]{0.3125\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/CS/frankfurt_000001_072295_leftImg8bit_texture_pred.png}
            \caption*{texture expert (T+C) prediction}
        \end{subfigure} %
        \begin{subfigure}[b]{0.3125\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/CS/frankfurt_000001_072295_leftImg8bit_anisodiff_pred.png}
            \caption*{shape expert (S+C) prediction}
        \end{subfigure} %
        \begin{subfigure}[b]{0.355\textwidth}
            \centering
            \def\svgwidth{\textwidth}
            \tiny
            \import{figures/fusion/texture_shape_visuals/CS/}{heatmap_PuBuGn_contour_anisodiff_CS19_deeplabv3resnet18_512x512_pseudoVal_1gpag6aw_2023_09_15_frankfurt_000001_072295.pdf_tex}
            \caption*{heatmap for shape influence}
        \end{subfigure}\\
    
        % \vspace{0.3cm}
        \begin{subfigure}[b]{0.3125\textwidth} %325
            \centering
            \includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/CS/frankfurt_000001_072295_leftImg8bit.png}
            \caption*{input image}
        \end{subfigure}  %
        \begin{subfigure}[b]{0.3125\textwidth} %325
            \centering
            \includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/CS/frankfurt_000001_072295_leftImg8bit_fusion_pred.png}
            \caption*{prediction of fusion model}
        \end{subfigure}  %
        \begin{subfigure}[b]{0.3125\textwidth} %325
            \centering
            \includegraphics[width=\textwidth, trim=0 0 10 0, clip]{figures/fusion/texture_shape_visuals/CS/frankfurt_000001_072295_gtFine_color.png}\hfill%
            \caption*{ground truth}
        \end{subfigure}
    \end{minipage}
    \caption[Comparison between expert prediction and late fusion prediction]{A visual example of the predictions of an S+C and a T+C expert as well as the fusion model of an Cityscapes image. This is complemented with a heatmap depicting the pixel-wise input-dependent weighting for shape. Consequently, in lighter areas the texture cue is dominating.}\label{fig:cityscapes_fusion}
\end{figure*}


==> figures/fusion/fig_zz_overview_fusion_pred_heat.tex <==
\begin{figure}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/CS/frankfurt_000001_072295_leftImg8bit_texture_pred.png}
        \caption*{texture expert (T+C) prediction}
    \end{subfigure} %
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/CS/frankfurt_000001_072295_leftImg8bit_anisodiff_pred.png}
        \caption*{shape expert (S+C) prediction}
    \end{subfigure} %
    \begin{subfigure}[b]{0.3425\textwidth}
        \centering
        \def\svgwidth{\textwidth}
        \tiny
        \import{figures/fusion/texture_shape_visuals/CS/}{heatmap_PuBuGn_contour_anisodiff_CS19_deeplabv3resnet18_512x512_pseudoVal_1gpag6aw_2023_09_15_frankfurt_000001_072295.pdf_tex}
        \caption*{heatmap for shape influence}
    \end{subfigure}

    \vspace{0.3cm}
    \begin{subfigure}[b]{0.3\textwidth} %325
        \centering
        \includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/CS/frankfurt_000001_072295_leftImg8bit.png}
        \caption*{input image}
    \end{subfigure}  %
    \begin{subfigure}[b]{0.3\textwidth} %325
        \centering
        \includegraphics[width=\textwidth]{figures/fusion/texture_shape_visuals/CS/frankfurt_000001_072295_leftImg8bit_fusion_pred.png}
        \caption*{prediction of fusion model}
    \end{subfigure}  %
    \begin{subfigure}[b]{0.3\textwidth} %325
        \centering
        \includegraphics[width=\textwidth, trim=0 0 10 0, clip]{figures/fusion/texture_shape_visuals/CS/frankfurt_000001_072295_gtFine_color.png}\hfill%
        \caption*{ground truth}
    \end{subfigure}
    \caption[Comparison between expert prediction and late fusion prediction]{A visual example of the predictions of an S+C and a T+C expert as well as the fusion model of an Cityscapes image. This is complemented with a heatmap depicting the pixel-wise input-dependent weighting for shape. Consequently, in lighter areas the texture cue is dominating.}\label{fig:cityscapes_fusion}
\end{figure}

